Socially Responsible Data for Large Multilingual Language Models

Large Language Models (LLMs) have rapidly increased in size and apparent capabilities in the last three years, but their training data is largely English text. There is growing interest in multilingual LLMs, and various efforts are striving for models to accommodate languages of communities outside of the Global North, which include many languages that have been historically underrepresented in digital realms. These languages have been coined as "low resource languages" or "long-tail languages", and LLMs performance on these languages is generally poor. While expanding the use of LLMs to more languages may bring many potential benefits, such as assisting cross-community communication and language preservation, great care must be taken to ensure that data collection on these languages is not extractive and that it does not reproduce exploitative practices of the past. Collecting data from languages spoken by previously colonized people, indigenous people, and non-Western languages raises many complex sociopolitical and ethical questions, e.g., around consent, cultural safety, and data sovereignty. Furthermore, linguistic complexity and cultural nuances are often lost in LLMs. This position paper builds on recent scholarship, and our own work, and outlines several relevant social, cultural, and ethical considerations and potential ways to mitigate them through qualitative research, community partnerships, and participatory design approaches. We provide twelve recommendations for consideration when collecting language data on underrepresented language communities outside of the Global North.

==> recTable.tex <==
\begin{table}[]
    \centering \footnotesize
    \begin{tabularx}{\textwidth}{ 
  | >{\flushleft\arraybackslash}X 
  | >{\flushleft\arraybackslash}X | }
        \hline 
        {\bf Recommendation} & {\bf Description} \\
        \hline
         1) \textbf{Respect the Autonomy of Local Communities} &  We implore researchers to respect the rights of local communities in their decisions regarding the necessity of Large Language Models (LLMs) in their language, avoiding any imposition of Western or colonial perspectives \cite{bird2020decolonising} \\ \hline
         2) \textbf{Critical Examination of Data Projects} & It is crucial to critically assess their potential ramifications to ensure the welfare of the affected communities when collecting or processing data. This entails an examination of power dynamics, implicit biases, and contextual factors that may introduce inequity \cite{schwartz2022primum} \\ \hline
         3) \textbf{Engage Local Communities as Partners} & Embrace ethnographic methods to engage with local communities as partners in data collection endeavors. This approach, especially when working with communities that share a common language with researchers, fosters trust and facilitates the development of beneficial technologies \cite{bird2020decolonising}. \\ \hline         
         4) \textbf{Ensure Accurate Language Representation} & Dedicate the necessary time and resources to ensure accurate representation of languages in the work. \\ \hline
         5) \textbf{Understand Local Technology Needs} & Recognize and address local technology needs, which may include language revitalization, preservation, migration challenges, and cross-community communication. \\ \hline
         6) \textbf{Acknowledge Global and Local Power Relations} & Investigate the power dynamics within the local context and how they influence access to language-based technologies, data collection, and the potential impact of LLMs on these power relations. \\ \hline
         7) \textbf{Incorporate Intersectionality and Qualitative Approaches} & Apply justice-oriented intersectionality theory and qualitative approaches to data collection. Consider how layers of identity affect individuals' lived experiences, power dynamics, and marginalization \cite{collins2020intersectionality, davis2021algorithmic, kapania2023hunt}. \\
         \hline
         8) \textbf{Transfer LLM Technology to Global South Stakeholders} & Promote the transfer of LLM technology to stakeholders in the Global South. This includes giving local stakeholders agency in determining approaches and annotator inclusion \cite{bird2020decolonising}. \\ \hline
         9) \textbf{Implement Data Governance} & Embrace concepts of data governance throughout the research process, including data collection. Clarify ownership and decision-making, recognizing that open-source does not equate to community-owned data. \\ \hline
         10) \textbf{Support Community-Based Language Intiatives} & Extend support to existing community-based language projects---Māori data sovereignty, Masakhane (“we build together”) and alike, which emphasize collaborative efforts \cite{bird2022local}. \\ \hline
        11) \textbf{Value Community Empowerment} & Prioritize data collection processes that bring cultural and economic value to the community. Acknowledge that marginalized communities may have different perspectives on language and knowledge work compared to Western researchers \cite{bird2022local}. \\ \hline
        12) \textbf{Engage with Local Community Concerns} & When developing bias and safety evaluation datasets, collaborate with the local community to understand and address local cultural concerns and stereotypes \cite{dev2023building}. \\ \hline
        
    \end{tabularx}
    \caption{Recommendations for socially responsible language data collection for underserved language communities}
    \label{tab:sources}
\end{table}

==> table.tex <==
\begin{landscape}

\begin{table}[ht]
  \caption{Recommendations for socially responsible language data collection for underserved language communities.}
  \label{tab:freq}
   \begin{tabular}{>{\raggedright\arraybackslash}m{10mm}|m{50mm}|m{120mm}}
   \hline
   \multicolumn{1}{>{\centering\arraybackslash}m{10mm}|}{\textbf{Num}} 
    & \multicolumn{1}{>{\centering\arraybackslash}m{50mm}|}{\textbf{Recommendation}} 
    & \multicolumn{1}{>{\centering\arraybackslash}m{120mm}}{\textbf{Description}}\\
    \hline

    1 & \textsl{Respect the Autonomy of Local Communities} & We implore researchers to respect the rights of local communities in their decisions regarding the necessity of Large Language Models (LLMs) in their language, avoiding any imposition of Western or colonial perspectives \cite{bird2020decolonising}. \\ 
    
    \hline
    
    2 & \textsl{Critical Examination of Data Collection Projects} & Prior to embarking on data collection initiatives, it is crucial to critically assess their potential ramifications to ensure the welfare of the affected communities. This entails an examination of power dynamics, implicit biases, and contextual factors that may introduce inequity \cite{schwartz2022primum}.\\
    \hline
    
    3 & \textsl{Engage Local Communities as Partners} & Embrace ethnographic methods to engage with local communities as partners in data collection endeavours. This approach, especially when working with communities that share a common language with researchers, fosters trust and facilitates the development of beneficial technologies \cite{bird2020decolonising}. \\
    \hline
    4 & \textsl{Ensure Accurate Language Representation} & Dedicate the necessary time and resources to ensure accurate representation of languages in the work.  \\
    \hline
    
    5 & \textsl{Understand Local Technology Needs} & Recognize and address local technology needs, which may include language revitalization, preservation, migration challenges, and cross-community communication \cite{cooper2024, bird2022local}. \\ 
    \hline
    
    6 & \textsl{Acknowledge Local Power Relations} & Investigate the power dynamics within the local context and how they influence access to language-based technologies, data collection, and the potential impact of LLMs on these power relations. \\ 
    
    \hline
    7 & \textsl{Incorporate Intersectionality and Qualitative Approaches} & Apply justice-oriented intersectionality theory and qualitative approaches to data collection. Consider how layers of identity affect individuals' lived experiences, power dynamics, and marginalization \cite{collins2020intersectionality, davis2021algorithmic, kapania2023hunt}.\\ 
    \hline
    8 & \textsl{Transfer LLM Technology to Global South Stakeholders} & Promote the transfer of LLM technology to stakeholders in the Global South. This includes giving local stakeholders agency in determining approaches and annotator inclusion \cite{bird2020decolonising}. \\
    \hline
    9 & \textsl{Implement Data Governance} & Embrace concepts of data governance throughout the research process, including data collection. Clarify ownership and decision-making, recognizing that open-source does not equate to community-owned data. \\ 
    \hline
    10 & \textsl{Support Community-Based Language Initiatives} & Extend support to existing community-based language projects such as Māori data sovereignty, Masakhane (“we build together”) and alike, which emphasize collaborative efforts \cite{bird2022local}. \\
    \hline
    11 & \textsl{Value Community Empowerment} & Prioritize data collection processes that bring cultural and economic value to the community \cite{cooper2024}. Acknowledge that marginalized communities may have different perspectives on language and knowledge work compared to Western researchers \cite{bird2022local}. \\ 
    \hline
    12 & \textsl{Engage with Local Community Concerns} & When developing bias and safety evaluation datasets, collaborate with the local community to understand and address local cultural concerns and stereotypes \cite{dev2023building}. \\ 
    
  \bottomrule
\end{tabular}
\label{tab:Recs}
%\end{adjustbox}
\end{table}

\end{landscape}

